A Diffusion Model Translator for Efficient Image-to-Image Translation

Applying diffusion models to image-to-image translation (I2I) has recently received increasing attention due to its practical applications. Previous attempts inject information from the source image into each denoising step for an iterative refinement, thus resulting in a time-consuming implementation. We propose an efficient method that equips a diffusion model with a lightweight translator, dubbed a Diffusion Model Translator (DMT), to accomplish I2I. Specifically, we first offer theoretical justification that in employing the pioneering DDPM work for the I2I task, it is both feasible and sufficient to transfer the distribution from one domain to another only at some intermediate step. We further observe that the translation performance highly depends on the chosen timestep for domain transfer, and therefore propose a practical strategy to automatically select an appropriate timestep for a given task. We evaluate our approach on a range of I2I applications, including image stylization, image colorization, segmentation to image, and sketch to image, to validate its efficacy and general utility. The comparisons show that our DMT surpasses existing methods in both quality and efficiency. Code will be made publicly available.

==> TPAMI/0.abs.tex <==
\begin{abstract}


Applying diffusion models to image-to-image translation (I2I) has recently received increasing attention due to its practical applications.
%
Previous attempts inject the information from the source image into \textbf{each} denoising step for an iterative refinement, leading to time-consuming implementation.
%
We propose an efficient method that equips a diffusion model with a lightweight translator, dubbed a Diffusion Model Translator (\method), to accomplish I2I. 
%
Specifically, we first provide theoretical justification that, when using the pioneer DDPM work to accomplish the I2T task, it is feasible and sufficient to transfer the distribution from one domain to another only at \textbf{some intermediate} step.
%
We then observe that the translation performance highly depends on the selected timestep to perform domain transfer, and therefore propose a practical strategy to automatically select an appropriate timestep for a given task.
%
We evaluate our approach on a range of I2I applications, namely, image stylization, image colorization, segmentation to image, and sketch to image, to validate its efficacy and general utility.
%
Comparisons show that our \method surpasses existing methods in both quality and efficiency.
%
Code will be made publicly available.

% Applying diffusion models to image-to-image translation (I2I) has recently received wide attention due to its practical applications. Previous attempts inject the information from the source image into \textbf{each} denoising step for an iterative refinement, leading to time-consuming implementation. We propose an efficient method that equips a diffusion model with a lightweight translator, dubbed a Diffusion Model Translator (DMT), to accomplish I2I. Specifically, We first provide theoretical justification that, when using the DDPM to accomplish the I2T task, it is feasible and sufficient to transfer the distribution from one domain to another only at \textbf{some intermediate} step. We then observe that the translation performance highly depends on the selected timestep to perform domain transfer, and therefore propose a practical strategy to automatically select an appropriate timestep for a given task. We evaluate our approach on a range of I2I applications, namely, image stylelization, image colorization, segmentation to image, and sketch to image, to validate its efficacy and general utility. Comparisons show that DMT surpasses existing methods in both quality and efficiency. Code will be made publicly available.

\end{abstract}

==> figures/difficulty/fig.tex <==
\begin{figure*}[h]
\centering
\includegraphics[width=0.8\linewidth]{figures/difficulty/difficulty_all.pdf}
\vspace{-15pt}
\caption{
    \textbf{Conceptual illustration} of the minimum of $C(S)=\max\{f(t),g(t)\}$ at the timestep $t^*$, which corresponds to the intersection of two curves $f(t)$ and $g(t)$.
}
\label{fig:difficulty}
%\vspace{-10pt}
\end{figure*}

==> figures/fig_ablation_t_afhq_rebuttal/fig.tex <==
% \definecolor{myblue}{RGB}{132, 180, 213}
% \definecolor{myred}{RGB}{213, 123, 101}
\definecolor{myblue}{RGB}{0, 0, 0}
\definecolor{myred}{RGB}{0, 0, 0}
\begin{figure*}[tp]
\centering
\begin{tabular}{ccc}
\begin{minipage}[t]{0.3\linewidth}\includegraphics[width=1\linewidth]{figures/fig_ablation_t_afhq_rebuttal/afhq_metric_L1.png}\end{minipage} &
\begin{minipage}[t]{0.3\linewidth}\includegraphics[width=1\linewidth]{figures/fig_ablation_t_afhq_rebuttal/afhq_metric_L2.png}\end{minipage} &
\begin{minipage}[t]{0.3\linewidth}\includegraphics[width=1\linewidth]{figures/fig_ablation_t_afhq_rebuttal/afhq_metric_SSIM.png}\end{minipage} \\
(a) $L_1$ & (b) $L_2$ & (c) SSIM \\
\begin{minipage}[t]{0.3\linewidth}\includegraphics[width=1\linewidth]{figures/fig_ablation_t_afhq_rebuttal/afhq_metric_PSNR.png}\end{minipage} &
\begin{minipage}[t]{0.3\linewidth}\includegraphics[width=1\linewidth]{figures/fig_ablation_t_afhq_rebuttal/afhq_metric_FID.png}\end{minipage} &
\begin{minipage}[t]{0.3\linewidth}\includegraphics[width=1\linewidth]{figures/fig_ablation_t_afhq_rebuttal/afhq_metric_LPIPS.png}\end{minipage} \\
(d) PSNR & (e) FID & (f) LPIPS
\end{tabular}
\caption{
    \textbf{Analysis on the preset timestep, $t$.}
    %
    We introduce 6 distinct metrics, \textit{i.e.}, $L_1$, $L_2$, SSIM, PSNR, FID, and LPIPS.
    %
    We plot the distance between $(x_t,y_t)$ and $(x_0, x_t)$ at different timesteps on AFHQ dataset, which are shown in red and blue curves, respectively.
}
\label{fig:ablation_t_afhq}
\vspace{-10pt}
\end{figure*}



==> figures/fig_ablation_t_celebahq_rebuttal/fig.tex <==
% \definecolor{myblue}{RGB}{132, 180, 213}
% \definecolor{myred}{RGB}{213, 123, 101}
\definecolor{myblue}{RGB}{0, 0, 0}
\definecolor{myred}{RGB}{0, 0, 0}
\begin{figure*}[tp]
\centering
\begin{tabular}{ccc}
\begin{minipage}[t]{0.3\linewidth}\includegraphics[width=1\linewidth]{figures/fig_ablation_t_celebahq_rebuttal/celebahq_metric_L1.png}\end{minipage} &
\begin{minipage}[t]{0.3\linewidth}\includegraphics[width=1\linewidth]{figures/fig_ablation_t_celebahq_rebuttal/celebahq_metric_L2.png}\end{minipage} &
\begin{minipage}[t]{0.3\linewidth}\includegraphics[width=1\linewidth]{figures/fig_ablation_t_celebahq_rebuttal/celebahq_metric_SSIM.png}\end{minipage} \\
(a) $L_1$ & (b) $L_2$ & (c) SSIM \\
\begin{minipage}[t]{0.3\linewidth}\includegraphics[width=1\linewidth]{figures/fig_ablation_t_celebahq_rebuttal/celebahq_metric_PSNR.png}\end{minipage} &
\begin{minipage}[t]{0.3\linewidth}\includegraphics[width=1\linewidth]{figures/fig_ablation_t_celebahq_rebuttal/celebahq_metric_FID.png}\end{minipage} &
\begin{minipage}[t]{0.3\linewidth}\includegraphics[width=1\linewidth]{figures/fig_ablation_t_celebahq_rebuttal/celebahq_metric_LPIPS.png}\end{minipage} \\
(d) PSNR & (e) FID & (f) LPIPS
\end{tabular}
\caption{
    \textbf{Analysis on the preset timestep, $t$.}
    %
    We introduce 6 distinct metrics, \textit{i.e.}, $L_1$, $L_2$, SSIM, PSNR, FID, and LPIPS.
    %
    We plot the distance between $(x_t,y_t)$ and $(x_0, x_t)$ at different timesteps on CelebA-HQ dataset, which are shown in red and blue curves, respectively.
}
\label{fig:ablation_t_celebahq}
\vspace{-10pt}
\end{figure*}



==> figures/fig_comparison/fig_response.tex <==
\begin{figure*}[!ht]
\centering
%\setlength\tabcolsep{2pt}
%\begin{tabular}{cc}
%\begin{minipage}[t]{0.55\linewidth}\includegraphics[width=1\linewidth]{figures/fig_method/method_palette.pdf}\end{minipage} &
%\begin{minipage}[t]{0.45\linewidth}\includegraphics[width=1\linewidth]{figures/fig_method/method_dmt.pdf}\end{minipage} \\
%(a) Our proposed \method & (b) Palette
%\end{tabular}
\includegraphics[width=0.98\textwidth]{figures/fig_comparison/comparison_highlight_nored.pdf}
\vspace{-5pt}
\caption{
    \textbf{Qualitative comparison}. Our \method achieves on par or better results than the three baseline methods Pix2Pix, Palette, TSIT on the four I2I tasks, \sqq{which are} image stylization, image colorization, segmentation to image, and sketch to image. Significant differences are highlighted in red or blue boxes, and brief textual explanations are provided \yr{besides the boxes}.
}
\label{fig:comparison}
\vspace{-5pt}
\end{figure*}


==> figures/fig_comparison_sd/fig.tex <==
\begin{figure*}[!ht]
\centering
\includegraphics[width=0.98\textwidth]{figures/fig_comparison_sd/comparison_sd.pdf}
\vspace{-15pt}
\caption{
    \textbf{Qualitative comparison}.
    %
    One can observe that both Pix2Pix~\cite{isola2017image} and TSIT~\cite{jiang2020tsit} backbones fail to handle the domain shift on colorization and segmentation-to-image tasks on latent space based on Stable Diffusion (SD)~\cite{Rombach2021HighResolutionIS}, leading to bad performance of our \method.
    %
    That is to say, existing attemps on I2I is not designed to be applied on latent spaces.
    %
    As a comparison, \method on pixel space shows extremely high synthesis quality.
}
\label{fig:comparison_sd}
\vspace{-5pt}
\end{figure*}


==> figures/fig_ddpm-dmt/fig.tex <==
\begin{figure}[ht]
\vspace{-8pt}
\centering
%\setlength\tabcolsep{2pt}
%\begin{tabular}{cc}
%\begin{minipage}[t]{0.55\linewidth}\includegraphics[width=1\linewidth]{figures/fig_method/method_palette.pdf}\end{minipage} &
%\begin{minipage}[t]{0.45\linewidth}\includegraphics[width=1\linewidth]{figures/fig_method/method_dmt.pdf}\end{minipage} \\
%(a) Our proposed \method & (b) Palette
%\end{tabular}
\includegraphics[width=0.45\textwidth]{figures/fig_ddpm-dmt/fig_new.pdf}
% \vspace{-10pt}
% \caption{
%     \textbf{Qualitative} comparison.
% }
\label{fig:ddpm-dmt}
\vspace{-10pt}
\end{figure}


==> tables/ablation_s_t.tex <==
\setlength{\tabcolsep}{10pt}
\begin{table*}[t]
% \renewcommand\arraystretch{1.2}
\centering
\caption{
    \textbf{Ablation study} on the preset timestep pair $(s,t)$ in our proposed \method on the two I2I tasks under different $\lambda$ defined in \cref{eq:s_t}.
    %
    SSIM is used to evaluate the distance between samples.
}
\label{tab:ablation_s_t}
\vspace{-2pt}
\begin{tabular}{l|ccc}
\toprule
             &      $\lambda=0.1$ &     $\lambda=0.25$ &      $\lambda=0.5$ \\
\midrule
 Stylization &   $(s,t)=(50, 50)$ &   $(s,t)=(50, 50)$ &   $(s,t)=(50, 50)$ \\
Colorization &      $(s,t)=(5,5)$ &      $(s,t)=(5,5)$      & $(s,t)=(5,5)$ \\
Segmentation & $(s,t)=(200, 400)$ & $(s,t)=(200, 400)$ & $(s,t)=(200, 200)$ \\
      Sketch &   $(s,t)=(20, 20)$ &   $(s,t)=(20, 20)$ &   $(s,t)=(20, 20)$ \\
\bottomrule
\end{tabular}
\end{table*}



==> tables/ablation_s_t_quan.tex <==
\setlength{\tabcolsep}{10pt}
\begin{table*}[t]
% \renewcommand\arraystretch{1.2}
\centering
\caption{
    \textbf{Quantitative comparison} between the identical and asymmetric timestep for domain shift by \method.
    %
    Both pipelines are trained upon the TSIT~\cite{jiang2020tsit} backbone on CelebA-HQ dataset for segmentation to image task.
}
\label{tab:ablation_s_t_quan}
\vspace{-2pt}
\begin{tabular}{l|ccc}
\toprule
                               & \textbf{FID$\downarrow$} & \textbf{SSIM$\uparrow$} & \textbf{LPIPS$\downarrow$} \\
\midrule
Identical, $t=200$             &                \bf 36.78 &               \bf 0.446 &                  \bf 0.433 \\
Asymmetric, $(s,t)=(200,400) $ &                    53.42 &                   0.328 &                      0.493 \\
\bottomrule
\end{tabular}
\end{table*}



==> tables/ablation_t_rebuttal.tex <==
\setlength{\tabcolsep}{8pt}
\begin{table*}[!ht]
\footnotesize
% \renewcommand\arraystretch{1.2}
\centering
\caption{
    \textbf{Quantitative comparison} of \method upon TSIT~\cite{jiang2020tsit} at different timesteps determined by different metrics.
    %
    FID are SSIM are used to evaluate the image quality and content preservation, respectively.
}
\label{tab:ablation_t_rebuttal}
\vspace{-2pt}
\begin{tabular}{l|ccc|ccc}
\toprule
       & \multicolumn{3}{c|}{Colorization} & \multicolumn{3}{c|}{Segmentation} \\
\midrule
Metric  & $t^*$ & \textbf{FID$\downarrow$} & \textbf{SSIM$\uparrow$} & $t^*$ & \textbf{FID$\downarrow$} & \textbf{SSIM$\uparrow$} \\
\midrule
                        $L_1$ & 50 &     15.18 &     0.496 & 200 & \bf 36.78 &     0.446 \\
                        $L_2$ & 50 &     15.18 &     0.496 & 200 & \bf 36.78 &     0.446 \\
\rowcolor{lightgray!30} SSIM  &  5 & \bf 13.03 & \bf 0.684 & 200 & \bf 36.78 &     0.446 \\
                        PSNR  & 50 &     15.18 &     0.496 & 200 & \bf 36.78 &     0.446 \\
                        FID   & 50 &     15.18 &     0.496 & 200 & \bf 36.78 &     0.446 \\
                        LPIPS &  5 & \bf 13.03 & \bf 0.684 & 100 &     37.22 & \bf 0.460 \\
\bottomrule
\end{tabular}
\end{table*}



==> tables/ablation_t_star_afhq.tex <==
\begin{table}[ht]
\small
\renewcommand\arraystretch{1}
\centering
\vspace{-8pt}
\caption{
    \textbf{Ablation study} of $t$ near $t^*$ on AFHQ dataset.
}
\label{tab:ablation_t_star_afhq}
\vspace{-10pt}
\begin{tabular}{l|ccccc}
\toprule
$t$ & 0 & 5 ($t^*$) & 10 & 15 & 25 \\
\midrule
\bf FID$\downarrow$ & 13.28 & \textbf{13.03} & 13.61  & 13.92  & 14.62  \\
\bf SSIM$\uparrow$  & \textbf{0.708} & 0.684 & 0.680  & 0.620  & 0.537  \\
\bottomrule
\end{tabular}
%\vspace{-12pt}
\end{table}

==> tables/ablation_t_star_celebahq.tex <==
\begin{table}[ht]
\small
\renewcommand\arraystretch{1}
\centering
\vspace{-8pt}
\caption{
    \textbf{Ablation study} of $t$ near $t^*$ on CelebA-HQ dataset.
}
\label{tab:ablation_t_star_celebahq}
\vspace{-10pt}
\begin{tabular}{l|ccccccc}
\toprule
$t$                 &   180 &   190 &       195 & 200 ($t^*$) &   205 &   210 &       220 \\
\midrule
\bf FID$\downarrow$ & 37.93 & 38.48 &     36.46 &       36.78 & 37.09 & 39.62 & \bf 36.04 \\
\bf SSIM$\uparrow$  & 0.450 & 0.438 & \bf 0.455 &       0.446 & 0.420 & 0.418 &     0.432 \\
\bottomrule
\end{tabular}
% \vspace{-12pt}
\end{table}

==> tables/comparison_sd.tex <==
\setlength{\tabcolsep}{8pt}
\begin{table*}[!ht]
\footnotesize
% \renewcommand\arraystretch{1.2}
\centering
\caption{
    \textbf{Quantitative comparison} between Pix2Pix~\cite{isola2017image}, TSIT~\cite{jiang2020tsit} and our proposed \method upon Stable Diffusion (SD)~\cite{Rombach2021HighResolutionIS}, and pixel space.
    %
    We introduce the Stable Diffusion V1.4, encoding the images into latent codes and denoising the noisy intermediate results into pure data samples.
    %
    FID, SSIM and LPIPS are used to evaluate the image quality and content preservation, respectively.
}
\label{tab:quantitative_comparison_sd}
\vspace{-2pt}
\begin{tabular}{l|cccc|cccc}
\toprule
       & \multicolumn{4}{c|}{Colorization} & \multicolumn{4}{c|}{Segmentation} \\
\midrule
Method  & \textbf{FID$\downarrow$} & \textbf{SSIM$\uparrow$} & \textbf{LPIPS$\downarrow$} & \textbf{Epoch} & \textbf{FID$\downarrow$} & \textbf{SSIM$\uparrow$} & \textbf{LPIPS$\downarrow$} & \textbf{Epoch} \\
\midrule
Pix2Pix                       &    108.54 &     0.168 &     0.649 &   60 &    119.77 &     0.115 &     0.686 & 60 \\
Pix2Pix-\method (Ours, SD)    &     71.00 &     0.177 &     0.654 &   60 &    125.60 &     0.130 &     0.643 & 60 \\
Pix2Pix-\method (Ours, pixel) & \bf 17.44 & \bf 0.752 & \bf 0.263 &   60 & \bf 65.26 & \bf 0.137 & \bf 0.534 & 60 \\
\midrule
TSIT                          &    220.20 &     0.098 &     0.729 &   60 &    223.91 &     0.164 &     0.723 & 60 \\
TSIT-\method (Ours, SD)       &     89.25 &     0.084 &     0.646 &   60 &    101.36 &     0.260 &     0.583 & 60 \\
TSIT-\method (Ours, pixel)    & \bf 13.03 & \bf 0.684 & \bf 0.180 &   60 & \bf 36.78 & \bf 0.446 & \bf 0.433 & 60 \\
\bottomrule
\end{tabular}
\end{table*}



==> tables/ddpm-dmt.tex <==
\begin{table}[ht]
\small
\renewcommand\arraystretch{1}
\centering
% \vspace{-10pt}
% \caption{
%     \textbf{Quantitative} comparison.
% }
\label{tab:ddpm-dmt}
\vspace{-10pt}
\begin{tabular}{l|cccccc}
% \toprule
Method & \textbf{FID$\downarrow$} & \textbf{SSIM$\uparrow$} & \textbf{LPIPS$\downarrow$} & \textbf{L1$\downarrow$} & \textbf{L2$\downarrow$} \\
\hline
DDPM-DMT & 108.07 & 0.590 & 0.317  & 0.162  & 0.059 \\
TSIT-DMT & \bf 64.97 & \bf 0.718 & \bf 0.225  & \bf 0.113  & \bf 0.027 \\
% \bottomrule
\end{tabular}
\vspace{-10pt}
\end{table}

==> tables/metric_anime.tex <==
\begin{table}[ht]
\small
\renewcommand\arraystretch{.4}
\centering
\vspace{-10pt}
\caption{
    Result on cartoonization task.
}
\label{tab:compare1}
\vspace{-10pt}
\begin{tabular}{l|cccc}
\toprule
%& \multicolumn{2}{c|}{Cartoonization}& \multicolumn{2}{c|}{Colorization} & \multicolumn{2}{c|}{Segmentation} & \multicolumn{2}{c|}{Sketches} \\
%\midrule
Method & \textbf{LPIPS$\downarrow$} & \textbf{L1$\downarrow$} & \textbf{L2$\downarrow$} & \textbf{user study$\uparrow$} \\
\midrule
Palette     & 0.386  & 0.281  & 0.154 & 0  \\
\midrule
Pix2Pix     & 0.277  & 0.108  & 0.038 & 0  \\
Pix2Pix-DMT & 0.259  & 0.106  & 0.029 & 0  \\
\midrule
TSIT        & 0.251  & 0.120  & 0.043 & 0  \\
TSTI-DMT    & 0.225  & 0.113  & 0.027 & 0  \\
\bottomrule
\end{tabular}
\end{table}


==> tables/metric_celeba.tex <==
\begin{table}[ht]
\small
\renewcommand\arraystretch{1}
\centering
% \vspace{-5pt}
% \caption{
%     \textbf{Quantitative} result on segmentation to image task.
% }
\label{tab:compare2}
\vspace{-8pt}
\begin{tabular}{l|cccccc}
% \toprule
%& \multicolumn{2}{c|}{Cartoonization}& \multicolumn{2}{c|}{Colorization} & \multicolumn{2}{c|}{Segmentation} & \multicolumn{2}{c|}{Sketches} \\
%\midrule
Method & \textbf{FID$\downarrow$} & \textbf{SSIM$\uparrow$} & \textbf{LPIPS$\downarrow$} & \textbf{L1$\downarrow$} & \textbf{L2$\downarrow$} & \textbf{Score$\uparrow$} \\
\hline
Palette     & 40.77 & 0.092 & 0.521  & 0.354  & 0.289 & 3.0  \\
\hline
Pix2Pix     & 70.98 & 0.105 & 0.542  & 0.448  & 0.351 & 1.7  \\
Pix2Pix-DMT & \bf 65.26 & \bf 0.137 & \bf 0.534  & \bf 0.427  & \bf 0.288 & \bf 3.5  \\
\hline
TSIT        & 40.59 & 0.357 & 0.450  & 0.194  & 0.072 & 3.6  \\
TSTI-DMT    & \bf 40.18 & \bf 0.437 & \bf 0.433  & \bf 0.182  & \bf 0.053 & \bf 4.4  \\
% \bottomrule
\end{tabular}
\vspace{-12pt}
\end{table}

